Highlights on top quark physics with the ATLAS experiment at the LHC

The large top-quark samples collected with the ATLAS experiment at the LHC have yielded measurements of the inclusive \ttbar production cross section of unprecedented precision and differential measurements in new kinematic regimes.They have also enabled new measurements of top-quark properties that were previously inaccessible, enabled the observation of many rare top-quark production processes predicted by the Standard Model and boosted searches for flavour-changing-neutral-current interactions of the top-quark, that are heavily suppressed in the SM. In this contribution the highlights of the ATLAS top-quark physics program are presented, as well as projections of the expected sensitivity after the High Luminosity phase of the LHC. Talk presented at the International Workshop on Future Linear Colliders (LCWS 2023), 15-19 May 2023. C23-05-15.3.

==> Makefile <==
# Makefile for creating an ATLAS LaTeX document

# Copyright (C) 2002-2023 CERN for the benefit of the ATLAS collaboration
#------------------------------------------------------------------------------
# By default makes mydocument.pdf using target run_pdflatex.
# Replace mydocument with your main filename or add another target set.
# Replace BIBTEX = biber with BIBTEX = bibtex if you use bibtex instead of biber.
# Adjust FIGSDIR for your figures directory tree.
# Adjust the %.pdf dependencies according to your directory structure.
# Use "make clean" to cleanup.
# Use "make cleanpdf" to delete $(BASENAME).pdf.
# "make cleanall" also deletes the PDF file $(BASENAME).pdf.
# Use "make cleanepstopdf" to remove PDF files created automatically from EPS files.
#   Note that FIGSDIR has to be set properly for this to work.

# Set the default target to run_pdflatex instead of run_latexmk to use explicit
# pdflatex/biber commands to compile.

# You can use the target version to check your TeX Live version.

#-------------------------------------------------------------------------------
# Check which TeX Live installation you have with the command pdflatex --version
PDFLATEX = pdflatex
# BIBTEX   = bibtex
BIBTEX   = biber
# TLVERS   = $(shell pdflatex --version | grep -Go 'TeX Live [0-9]*' | grep -Go '[0-9].*')
# TWIKI    = https://twiki.cern.ch/twiki/bin/view/AtlasProtected/PubComLaTeXFAQ

#-------------------------------------------------------------------------------
# The main document filename
BASENAME = mydocument

#-------------------------------------------------------------------------------
# Adjust this according to your top-level figures directory
# This directory tree is used by the "make cleanepstopdf" command
FIGSDIR  = figures
#-------------------------------------------------------------------------------

# EPSTOPDFFILES = `find . -name \*eps-converted-to.pdf`
rwildcard=$(foreach d,$(wildcard $1*),$(call rwildcard,$d/,$2) $(filter $(subst *,%,$2),$d))
EPSTOPDFFILES = $(call rwildcard, $(FIGSDIR), *eps-converted-to.pdf)

# Default target - make mydocument.pdf with latexmk.
default: run_latexmk
# Use pdflatex/biber instead to compile.
#default: run_pdflatex

.PHONY: run_latexmk
.PHONY: newdocument newdocumenttexmf newnotemetadata newpapermetadata newfiles
.PHONY: draftcover preprintcover newdata
.PHONY: version clean cleanpdf help

# Check TeX Live version
# version:
# 	@echo "Checking version"
# 	@echo "TLVERS $(TLVERS), TEXLIVE $(TEXLIVE)"
# 	@if [ $(TLVERS) -lt $(TEXLIVE) ]; then \
# 		echo "Your TeX Live version ($(TLVERS)) is older than $(TEXLIVE). Please consult $(TWIKI)"; \
# 	fi

# Standard pdflatex target
run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

# Remove -pdf option to run latex instead of pdflatex
run_latexmk:
	latexmk -pdf $(BASENAME)

#-------------------------------------------------------------------------------
# Specify the tex and bib file dependencies for running pdflatex
# If your bib files are not in the main directory adjust this target accordingly
%.pdf:	%.tex *.tex bib/*.bib
#%.pdf:	%.tex *.tex *.bib
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<
#-------------------------------------------------------------------------------

# Default is to make a new paper
new: newnote

newpaper: newdocument newfiles newpapermetadata newauxmat

clean:
	-rm *.toc *.aux *.lof *.lot *.log *.out \
		*.bbl *.blg *.brf *.bcf *-blx.bib *.run.xml \
		*.cb *.ind *.idx *.ilg *.inx *.tdo \
		*.synctex.gz *~ *.fls *.fdb_latexmk .*.lb spellTmp

cleanpdf:
	-rm $(BASENAME).pdff

cleanall: clean cleanpdf

==> mydocument-metadata.tex <==
%-------------------------------------------------------------------------------
% This file contains the title, author and abstract.
% It also contains all relevant document numbers used for an ATLAS note.
%-------------------------------------------------------------------------------

% Title
\title{Highlights on top quark physics with \\ the ATLAS experiment at the LHC}
% Abstract - % directly after { is important for correct indentation.
\abstract{%
The large top quark samples collected with the ATLAS experiment at the LHC have yielded measurements of the inclusive \ttbar production cross section of unprecedented precision and differential measurements in new kinematic regimes. 
They have also enabled new measurements of top quark properties that were previously inaccessible, enabled the observation of many rare top quark production processes predicted by the Standard Model and boosted searches for flavour-changing-neutral-current interactions of the top quark, that are heavily suppressed in the SM. 
In this contribution the highlights of the ATLAS top quark physics program are presented, as well as projections of the expected sensitivity after the High Luminosity phase of the LHC.\\\\
Talk presented at the International Workshop on Future Linear Colliders (LCWS 2023), 15-19 May 2023. C23-05-15.3.}
% Author - this does not work with revtex (add it after \begin{document})
\author{Benedikt Gocke, on behalf of the ATLAS Collaboration}

